Discovering Emotion and Reasoning its Flip in Multi-Party Conversations using Masked Memory Network and Transformer

Efficient discovery of a speaker's emotional states in a multi-party conversation is significant to design human-like conversational agents. During a conversation, the cognitive state of a speaker often alters due to certain past utterances, which may lead to a flip in their emotional state. Therefore, discovering the reasons (triggers) behind the speaker's emotion-flip during a conversation is essential to explain the emotion labels of individual utterances. In this paper, along with addressing the task of emotion recognition in conversations (ERC), we introduce a novel task - Emotion-Flip Reasoning (EFR), that aims to identify past utterances which have triggered one's emotional state to flip at a certain time. We propose a masked memory network to address the former and a Transformer-based network for the latter task. To this end, we consider MELD, a benchmark emotion recognition dataset in multi-party conversations for the task of ERC, and augment it with new ground-truth labels for EFR. An extensive comparison with five state-of-the-art models suggests improved performances of our models for both tasks. We further present anecdotal evidence and both qualitative and quantitative error analyses to support the superiority of our models compared to the baselines.

==> tab-sp-3.tex <==
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
\multicolumn{1}{c|}{\textbf{\#}} & \multicolumn{1}{c|}{\textbf{Speaker}} & \multicolumn{1}{c|}{\textbf{Utterance}} & \multicolumn{1}{c|}{\textbf{Emotion}} & \multicolumn{1}{c}{\textbf{Trigger}} \\ \hline \hline
$1$ & Ross & This is my wedding. & neutral & 0 \\ \hline
$2$ & Monica & All right, y'know what? We really are late! Let's go! Let's go! Let's go!! & anger & 0 \\ \hline
$3$ & Ross & Fine. You'll-you'll watch it on video when we get back. & neutral & 0 \\ \hline
$4$ & Chandler & Here you go Phoebe! Here you go Phobo! Phewbedo! Phaybobo. & joy & 0 \\ \hline
$5$ & Phoebe & Thank you. & neutral & 0 \\ \hline
$6$ & Ross & All right, let's go! Bye, Pheebs! & joy & 0 \\ \hline
$7$ & Joey & Bye, Pheebs! London baby!! & joy & 1 \\ \hline
$8$ & Phoebe & Oh, do you need a hug? You don't have to bring me anything! & joy & 0 \\ \hline
\end{tabular}%
}
\caption{Example dialog from MELD-FR where five speakers are involved.}
\label{tab:dial_eg_sp_3}
\end{table}
